Stress Testing the Booters: Understanding and Undermining the Business of DDoS Services

DDoS-for-hire services, also known as booters, have commoditized DDoS attacks and enabled abusive subscribers of these services to cheaply extort, harass and intimidate businesses and people by knocking them offline. However, due to the underground nature of these booters, little is known about their underlying technical and business structure. In this paper we empirically measure many facets of their technical and payment infrastructure. We also perform an analysis of leaked and scraped data from three major booters---Asylum Stresser, Lizard Stresser and VDO---which provides us with an in-depth view of their customers and victims. Finally, we conduct a large-scale payment intervention in collaboration with PayPal and evaluate its effectiveness. Based on our analysis we show that these services are responsible for hundreds of thousands of DDoS attacks and identify potentially promising methods of increasing booters' costs and undermining these services.

==> sections/revenue_cost.tex <==
\section{Geography}

In order to understand where operators and subscribers are potentially located,
we use aggregated data provided to us by PayPal that was computed from all the accounts identified by PayPal as belonging to booter operators
and subscribers. This data did not include any scale on the number of booter and subscriber accounts included in the dataset. It was
computed by assigning the location for each account to the country from which the majority of their login's occured and computing the percentage of
accounts assigned to each country. In the case that an account did not have a majority of their logins' occuring in a single country
it was removed from the dataset. This accounted for 3\% of subscriber accounts and none of operator accounts. Also, IP addresses
for proxies, VPN services, hosting service and Tor were removed using a database from IP2Location~\cite{ip2proxy}.

Based on this information 44\% of the accounts used to accept payments for booters are potentially owned by someone in the United
States as shown in Table~\ref{operatorAccounts}. The subscriber locations are similar with nearly half of the accounts owned by someone
potentially located in the Unitied States and many of the remaining account owners geolocated to Western Europe based their IP
as shown in Table~\ref{operatorAccounts}.
There are many inherent limitations of this data which we cannot correct or quantify due to the highly aggregated nature of the data. 
These include the fact that
booter services create multiple accounts to replace ones that are limited by PayPal. Thus it might be the case that a few booter
services control a large number of the total accounts and are biasing the location and the same could hold for customers as well.
However, these locations match with much of the anecdotal information of this ecosystem including their preference for advertising
in English language based underground forums and customer's preference for using PayPal as a payment method over more traditional
virtual currencies, such as Webmoney which is more commonly used by Russian cybercriminals.
Assuming it is accurate, there is the potential for a meaningful undermining of the booter ecosystem by increased
law enforcement resources focused on this problem.

\begin{table}[H]
\small
\centering
\begin{tabular}{lrlr}
\hline
\multicolumn{2}{c}{Operator} & \multicolumn{2}{c}{Subscriber} \\
\hline
\bfseries CC & \bfseries \% & \bfseries CC & \bfseries \% \\
\hline
US & 44.06\% & US & 47.58\% \\
PK & 15.03\% & DE & 10.45\% \\
CA & 13.99\% & GB & 5.60\% \\
GB & 6.29\%  & NL & 4.87\% \\
AU & 3.15\% & RU & 4.81\% \\
\hline
\end{tabular}
\caption {Top country IP geolocations of logins for booter operator's and subscriber's PayPal accounts.}
\label{operatorAccounts}
\end{table}



%By enumerating the list of active paid users logging into the vdos-s.com during a month of crawling, we can estimate the revenue generated by this specific service. Compared to the other booters that we have been monitoring, this one seems to be among top high quality service providers. There are at least two more booters reporting both the total number of their users and the number of their paid users, I'm collecting these numbers and we can use them to estimate the revenue generated by these two booters as well.     

